Agile Development of Linux Schedulers with Ekiben

Kernel task scheduling is important for application performance, adaptability to new hardware, and complex user requirements. However, developing, testing, and debugging new scheduling algorithms in Linux, the most widely used cloud operating system, is slow and difficult. We developed Ekiben, a framework for high velocity development of Linux kernel schedulers. Ekiben schedulers are written in safe Rust, and the system supports live upgrade of new scheduling policies into the kernel, userspace debugging, and bidirectional communication with applications. A scheduler implemented with Ekiben achieved near identical performance (within 1% on average) to the default Linux scheduler CFS on a wide range of benchmarks. Ekiben is also able to support a range of research schedulers, specifically the Shinjuku scheduler, a locality aware scheduler, and the Arachne core arbiter, with good performance.

==> background.tex <==
%\section{Background}

%\subsection{Motivation}

- cfs, the default in linux, is cool as a default, but is lacking in some ways. there don't seem to be a lot of low level bugs, but there have been plenty of high level bugs. decade of wasted cores paper. cfs is not work conserving. it can't help that it's completely huge. it's like 6000 lines of code.

CFS's design is a reasonable default and works well for many of the tasks run on desktop or server machines.
If we have more knowledge about the specific use cases of a machine, we can instead choose to run schedulers that make more optimal decisions for those use cases. The Shinjuku scheduler~\cite{shinjuku} shows that for workloads composed of many very small tasks, fast preemption can lower average job completion time. The Arachne scheduler~\cite{arachne} gives better performance isolation and flexibility by allowing applications to define their own core policies based on their workloads. Nest~\cite{nest} improves performance and energy efficiency for jobs with fewer tasks than cores by reusing a few warm cores rather than spreading new tasks across many cold cores.
Because these schedulers do not need to be generic baselines that work well in all circumstances, they can potentially be much smaller and simpler than CFS.


%- cfs is a good baseline, but if we know what we're aiming for, we can do better, shinjuku shows us we can get better average job completion time for jobs with lots of small tasks if we do fast preemption for small tasks. arachne shows us we can do better if we allow things that know about the user programs to make their own decisions rather than trying to guess. nest shows us that for datacenter workloads, we can get better performance and energy use if we try to keep tasks on a few hot cores rather than spreading them out so much. and all with fewer lines of code the 11000 line behemoth that is cfs (ok next makes changes to cfs so maybe its not the best comparison)

==> figures/ekiben_api.tex <==
\begin{table*}[ht!]
%    \small
    \centering
    \begin{tabular}{l|l|l}
    \Xhline{4\arrayrulewidth}
        \textbf{API Function} & \textbf{Description} & \textbf{Default} \\
        \hline
        \texttt{get\_policy(\&self)} & Get the policy number. & None. \\
        \makecell[l]{\texttt{pick\_next\_task(\&self, ...,} \\ \texttt{\qquad sched: Option$\langle$Schedulable$\rangle$)}
            \\ \texttt{\qquad $\xrightarrow{}$ Option$\langle$Schedulable$\rangle$}}
            & Pick the next task for the CPU & Run nothing. \\
        \makecell[l]{\texttt{pnt\_err(\&self, ...,} \\ \texttt{\qquad sched: Schedulable)}} & Could not schedule chosen task & Do nothing. \\
        \texttt{task\_dead(\&self, pid)} & A task died. & Do nothing. \\
        \texttt{task\_blocked(\&self, ...) } & A task blocked. & Do nothing. \\
        \makecell[l]{\texttt{task\_wakeup(\&self, ..., } \\ \texttt{\qquad sched: Schedulable)}} & A task woke up. & Do nothing. \\
        \makecell[l]{\texttt{task\_new(\&self, ..., } \\ \texttt{\qquad sched: Schedulable)}} & There is a new task. & Do nothing. \\
        \makecell[l]{\texttt{task\_preempt(\&self, ..., } \\ \texttt{\qquad sched: Schedulable)}} & A task was preempted. & Do nothing. \\
        \texttt{task\_yield(\&self, ...)} & A task yielded. & Do nothing. \\
        \texttt{task\_departed(\&self, ...)} & A task left the scheduler. & Do nothing. \\
        \texttt{task\_affinity\_changed(\&self,..)} & Change task's allowed CPUs. & Do nothing. \\
        \texttt{task\_prio\_changed(\&self,..)} & Change task's priority. & Do nothing. \\
        %\texttt{task\_latched(\&self, ...)} & A task been latched to a CPU. & Do nothing. \\
        \texttt{task\_tick(\&self, ...)} & A timer has triggered. & Do nothing. \\
        \makecell[l]{\texttt{select\_task\_rq(\&self, ...)} \\ \texttt{\qquad $\xrightarrow{}$ i32}} & Choose the CPU for a task. & Pick CPU 0. \\
        \makecell[l]{\texttt{selected\_task\_rq(\&self, }\\ \texttt{\qquad sched: Schedulable)}} & Chose the CPU successfully. & Do nothing. \\
        \makecell[l]{\texttt{migrate\_task\_rq(\&self, ..., }\\ \texttt{\qquad sched: Schedulable)} \\ \texttt{\qquad $\xrightarrow{}$ Schedulable}} & A task is moving CPUs. & Do nothing. \\
        \makecell[l]{\texttt{balance(\&self, ...)} \\ \texttt{\qquad $\xrightarrow{}$ Option $\langle$u64$\rangle$}} & Rebalance tasks onto CPU. & Do nothing. \\
        \texttt{balance\_err(\&self, ...)} & Could not move the chosen task & Do nothing. \\
        \makecell[l]{\texttt{reregister\_prepare(\&mut self)} \\ \texttt{\qquad $\xrightarrow{}$ Option$\langle$TransferOut$\rangle$}} &
            Prepare for an upgrade. & Do nothing. \\
        \makecell[l]{\texttt{reregister\_init(\&mut self, } \\ \texttt{\qquad Option$\langle$TransferIn$\rangle$)}} &
            Initialize during an upgrade. & Do nothing. \\
        %\makecell[l]{\texttt{register\_queue(\&self,} \\ \texttt{RingBuffer}}
        \makecell[l]{\texttt{register\_queue(\&self, } \\ \texttt{\qquad RingBuffer$\langle$UserMessage$\rangle$) -> i32}} &
            Register a user to kernel hint queue. & None. \\
        \makecell[l]{\texttt{register\_reverse\_queue(\&self, } \\ \texttt{\qquad RingBuffer$\langle$RevMessage$\rangle$) -> i32}} &
            Register a kernel to user queue. & None. \\
        \texttt{enter\_queue(\&self, id: i32, ...)} & Check the user hint queue. & Do nothing.\\
        \makecell[l]{\texttt{unregister\_queue(\&self, id: i32) } \\ \texttt{\qquad $\xrightarrow{}$ RingBuffer$\langle$UserMessage$\rangle$)}} &
            Unregister the user to kernel hint queue. & None. \\
        \makecell[l]{\texttt{unregister\_rev\_queue(\&self, id: i32) } \\ \texttt{\qquad $\xrightarrow{}$ RingBuffer$\langle$RevMessage$\rangle$)}} &
            Unregister the kernel to user queue. & None. \\
        \texttt{parse\_hint(\&self, hint: UserMessage)} & Synchronously parse hint. & Do nothing.
    \end{tabular}
    \caption[The API of the EkibenScheduler Trait.]{The API of the EkibenScheduler Trait. This is the API that a scheduler module must implement to be loadable as an Ekiben scheduler. \todo{I propose leaving out about half of these and just showing a selection of the interface so we can save space}}
    \label{tab:ekiben_api}
\end{table*}
